First Observation of Heavy Baryons \Sigma_b and \Sigma_b^*

We report an observation of new bottom baryons produced in proton-antiproton collisions at the Tevatron. Using 1.1 fb^{-1} of data collected by the CDF II detector, we observe four \Lambda_b^0\pi^{\pm} resonances in the fully reconstructed decay mode \Lambda_b^0 \to \Lambda_c^+ \pi^-, where \Lambda_c^+ \to p K^- \pi^+. We interpret these states as the \Sigma_b^{(*)\pm} baryons and measure the following masses: m_{\Sigma_b^+} = 5807.8^{+2.0}_{-2.2}(stat.) \pm 1.7(syst.) MeV/c^2, m_{\Sigma_b^-} = 5815.2 \pm 1.0(stat.) \pm 1.7(syst.) MeV/c^2, and m(\Sigma_b^*) - m(\Sigma_b) = 21.2^{+2.0}_{-1.9}(stat.) ^{+0.4}_{-0.3}(syst.) MeV/c^2.

==> defs.tex <==
\RequirePackage{xspace}
\def\mum    {\ensuremath{\,\mu\rm m}\xspace}
\def\mm     {\ensuremath{\rm \,mm}\xspace}

\def\mtr    {\ensuremath{\rm \,m}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\Tesla {\ensuremath{{\rm\,T}}\xspace}
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}
\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
%\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~A~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
\newcommand{\jprc}      [1]  {\jprBase\ C~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpa}       [1]  {\zpBase\ A~{\bf #1}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}




\def\cdf2{CDF II}
\def\run2{Run II}

%
% Units of measure
%

\newcommand{\pt}{\ifmmode  p_{\rm T}%
                 \else%
                            \mbox{$p_{\rm{T}}$ }%
                 \fi%
                 }%

\newcommand{\lxy}{\ifmmode  L_{\rm xy}%
                 \else%
                            \mbox{$\rm{L}_{\rm{xy}}$}%
                 \fi%
                 }%


\newcommand{\jpsi}{\ifmmode  \rm{J}/\psi%
                 \else%
                            \mbox{$\rm{J}/\psi$}%
                 \fi%
                 }
\newcommand{\mev}{\ifmmode  {\rm MeV}%
                 \else%
                            \mbox{MeV}%
                 \fi%
                 }%

\newcommand{\Cascade}{\ifmmode  \Xi%
                 \else%
                            \mbox{$\Xi$}%
                 \fi%
                 }%


\newcommand{\om}{\ifmmode  \Omega%
                 \else%
                            \mbox{$\Omega$}%
                 \fi%
                 }%

\newcommand{\mevc}{\ifmmode {\rm MeV}/c%
                 \else%
                            \mbox{MeV}$/c$%
                 \fi%
                 }%

\newcommand{\mevcc}{\ifmmode {\rm MeV}/c^2%
                 \else%
                           \mbox{MeV}$/c^2$%
                 \fi%
                 }%
\newcommand{\gev}{\ifmmode {\rm GeV}%
                 \else%
                           \mbox{GeV}%
                 \fi%
                 }%

\newcommand{\gevc}{\ifmmode {\rm GeV}/c%
                 \else%
                           \mbox{GeV}$/c$%
                 \fi%
                 }%
\newcommand{\gevcc}{\ifmmode {\rm GeV}/c^2%
                 \else%
                           \mbox{GeV}$/c^2$%
                 \fi%
                 }%
\newcommand{\kev}{\ifmmode {\rm keV}%
                 \else%
                           \mbox{keV}%
                 \fi%
                 }%
\newcommand{\cm}{\ifmmode {\rm cm}%
                 \else%
                           \mbox{cm}%
                 \fi%
                 }%
\newcommand{\mkm}{\ifmmode \mu\rm{m}%
                 \else%
                           \mbox{$\mu$m}%
                 \fi%
                 }%

\newcommand{\um}{\ifmmode \mu\rm{m}%
                 \else%
                           \mbox{$\mu$m}%
                 \fi%
                 }%

\newcommand{\m}{\ifmmode \rm{m}%
                 \else%
                           m%
                 \fi%
                 }%

\newcommand{\tl}{\ifmmode \rm{T}%
                 \else%
                           \mbox{T}%
                 \fi%
                 }%

\newcommand{\dedx}{\ifmmode dE/dx%
                 \else%
                           \mbox{$dE/dx$}%
                 \fi%
                 }%

\newcommand{\tof}{\ifmmode \rm{ToF}%
                 \else%
                           \mbox{ToF}%
                 \fi%
                 }%

\newcommand{\lumi}{\ifmmode \rm{\cal{L}}%
                 \else%
                           \cal{L}%
                 \fi%
                 }%

\newcommand{\ee}{\ifmmode \rm{e}^+\rm{e}^-%
                 \else%
                          \mbox{$\rm{e}^+\rm{e}^-$}%
                 \fi%
                }%

\newcommand{\ct}{\ifmmode ct%
                 \else%
                         \mbox{$ct$}%
                 \fi%
                 }%

\newcommand{\cterr}{\ifmmode \sigma_{ct}%
                 \else%
                         \mbox{$\sigma_{ct}$}%
                 \fi%
                 }%

\newcommand{\mc}{эонте--ыарло}
\newcommand{\ra}{\rightarrow}
\newcommand{\hra}{\hookrightarrow}
\newcommand{\detarg}{детектор ARGUS}
\newcommand{\detarga}{детектора ARGUS}
\newcommand{\ka}{\mbox{$l_k=0$},\mbox{$l_K=1$}}
\newcommand{\kk}{\mbox{$l_k=1$},\mbox{$l_K=0$}}
%
% Particles:
%

\newcommand{\Lc}{\ifmmode  \Lambda_c^+
                 \else
                           \mbox{$\Lambda_c^+$}
                 \fi
                }

\newcommand{\Lcpi}{\ifmmode  \Lambda_c^+\pi^-
                 \else
                           \mbox{$\Lambda_c^+\pi^-$}
                 \fi
                }

\newcommand{\Br}{\ifmmode  {\cal B} 
                 \else
                           \mbox{${\cal B}+$}
                 \fi
                }

\newcommand{\Lcst}{\ifmmode  \Lambda_c^{*}
                 \else
                           \mbox{$\Lambda_c^*$}
                 \fi
                }

\newcommand{\Lbst}{\ifmmode  \Lambda_b^{*}
                 \else
                           \mbox{$\Lambda_b^*$}
                 \fi
                }

\newcommand{\Lb}{\ifmmode  \Lambda_b^0
                 \else
                           \mbox{$\Lambda_b^0$}
                 \fi
                }

\newcommand{\Sic}{\ifmmode  \Sigma_c
                 \else
                           \mbox{$\Sigma_c$}
                 \fi
                }

\newcommand{\Sib}{\ifmmode  \Sigma_b
                 \else
                           \mbox{$\Sigma_b$}
                 \fi
                }

\newcommand{\Sb}{\ifmmode  \Sigma_b
                 \else
                           \mbox{$\Sigma_b$}
                 \fi
                }
\newcommand{\piSb}{\ifmmode  \pi_{\Sigma_b}
                 \else
                           \mbox{$\pi_{\Sigma_b}$}
                 \fi
                }
\newcommand{\ptSb}{\ifmmode  \pt(\Sb)
                 \else
                           \mbox{$\pt(\Sb)$}
                 \fi
                }
\newcommand{\ptpiSb}{\ifmmode  \pt(\piSb)
                 \else
                           \mbox{$\pt(\piSb)$}
                 \fi
                }


\newcommand{\dsig}{\ifmmode |d_0/\sigma_{d_0}|
                 \else
                           \mbox{$|d_0/\sigma_{d_0}|$}
                 \fi
                }
\newcommand{\costhst}{\ifmmode \cos\theta^*
                 \else
                           \mbox{$\cos\theta^*$}
                 \fi
                }


\newcommand{\lm}{\ifmmode  \Lambda
                 \else
                           \mbox{$\Lambda$}
                 \fi
                }
\newcommand{\ks}{\ifmmode \rm{K}_S^0
                 \else
                           \mbox{$\rm{K}_S^0$}
                 \fi
                }

% Replaced by Petar, 11/4/2006:
%\newcommand{\rs}{Same Charge}
%\newcommand{\ws}{Opposite Charge}
\newcommand{\rs}{$\Lb\pi^-$}
\newcommand{\ws}{$\Lb\pi^+$}

\newcommand{\HaUE}{\mbox{hadronization}}


\newcommand{\lmc}{\Lambda_c^+}
\newcommand{\lmcst}{\Lambda_c^{*+}}
\newcommand{\lam}{\Lambda^0}
\newcommand{\lmcpi}{\Lambda^+_c \pi^+\pi^-}
\newcommand{\pkpi}{pK^-\pi^+}
\newcommand{\lampi}{\lam \pi^+}
\newcommand{\lamppi}{\lam \pi^+\pi^+\pi^-}
\newcommand{\pk}{p\bar{K}^0}
\newcommand{\pks}{p\ks}
\newcommand{\dec}{\lmc\ra \pkpi}
\newcommand{\chain}{\Lambda_c^{*+}\ra\lmc\pi^+\pi^-}
\newcommand{\sicpi}{\Sigma_c^{++}\pi^-}
\newcommand{\siczpi}{\Sigma_c^{0}\pi^+}
\newcommand{\sic}{\Sigma_c^}
\newcommand{\sicpl}{\Sigma_c^{++}}
\newcommand{\sicz}{\Sigma_c^{0}}

%\newcommand{\Sb}{\ifmmode \Sigma_b\else $\Sigma_b$\fi}
%\newcommand{\Lb}{\ifmmode \Lambda_b\else $\Lambda_b$\fi}

\newcommand{\BR}{\mathcal{B}}
                 
% these below for Young diagrams:

\newcommand{\cell}{\framebox(5,5){}}
\newcommand{\row}{\framebox(10,5){}}
\newcommand{\column}{\framebox(5,10){}}
\newcommand{\mixed}{
                    \begin{picture}(10,10)(0,0)
                      \put(0,-1.25){\row}
                      \put(0,-6.25){\column}
                    \end{picture}
                   }
\newcommand{\srow}{
                    \begin{picture}(15,5)(0,0)
                      \multiput(0,-1.25)(5.01,0){3}{\cell}
                    \end{picture}
                   }
\newcommand{\scolumn}{
                    \begin{picture}(5,15)(0,0)
                      \multiput(0,-1.25)(0,-5){3}{\cell}
                    \end{picture}
                   }
\newcommand{\drow}{
                    \begin{picture}(10,5)(0,0)
                      \multiput(0,-1.25)(5.01,0){2}{\cell}
                    \end{picture}
                   }
\newcommand{\dcolumn}{
                    \begin{picture}(5,10)(0,0)
                      \multiput(0,-1.25)(0,-5){2}{\cell}
                    \end{picture}
                   }
\newcommand{\single}{
                    \begin{picture}(5,5)(0,0)
                      \put(0,-1.25){\cell}
                    \end{picture}
                   }

\newcommand{\mat}{\left(\begin{array}{cc} -\sin{\theta} & \cos{\theta} \\
                                           \cos{\theta} & \sin{\theta}
                        \end{array} \right) }
\newcommand{\rmat}{\left(\begin{array}{cc} \cos{\theta} & \sin{\theta} \\
                                              -\sin{\theta} & \sin{\theta}
                        \end{array} \right) }














%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

